Parallel Distributional Prioritized Deep Reinforcement Learning for Unmanned Aerial Vehicles

This work presents a study on parallel and distributional deep reinforcement learning applied to the mapless navigation of UAVs. For this, we developed an approach based on the Soft Actor-Critic method, producing a distributed and distributional variant named PDSAC, and compared it with a second one based on the traditional SAC algorithm. In addition, we also embodied a prioritized memory system into them. The UAV used in the study is based on the Hydrone vehicle, a hybrid quadrotor operating solely in the air. The inputs for the system are 23 range findings from a Lidar sensor and the distance and angles towards a desired goal, while the outputs consist of the linear, angular, and, altitude velocities. The methods were trained in environments of varying complexity, from obstacle-free environments to environments with multiple obstacles in three dimensions. The results obtained, demonstrate a concise improvement in the navigation capabilities by the proposed approach when compared to the agent based on the SAC for the same amount of training steps. In summary, this work presented a study on deep reinforcement learning applied to mapless navigation of drones in three dimensions, with promising results and potential applications in various contexts related to robotics and autonomous air navigation with distributed and distributional variants.

==> sections/0_data_paper.tex <==
\title{Parallel Distributional Deep Reinforcement Learning for Drones}

\titlerunning{Parallel Distributional Deep Reinforcement Learning for Drones}

\thanks{$^{1}$Victor Augusto Kich, Alisson Henrique Kolling, and Daniel Fernando Tello Gamarra are with Federal University of Santa Maria, Brazil.
E-mail: {\tt\small victorkich@yahoo.com.br}
}
%
\thanks{$^{2}$ Ricardo Bedin Grando are with the Technological Unit, Techonological University of Uruguay -- UTEC, Rivera, Uruguay.
E-mail: {\tt\small ricard.bedin@utec.edu.uy}
}
%
\thanks{$^{3}$Junior Costa de Jesus and Paulo L. J. Drews-Jr are with the NAUTEC, Centro de Ciências Computacionais, Univ. Fed. do Rio Grande -- FURG, RS, Brazil.
E-mail: {\tt\small paulodrews@furg.br}
}

\author{Victor Augusto Kich$^{1}$, Alisson Henrique Kolling$^{1}$, Ricardo Bedin Grando$^{2}$, Junior Costa de Jesus$^{3}$, Paulo Lilles Jorge Drews-Jr$^{3}$, Daniel Fernando Tello Gamarra$^{1}$
}

\authorrunning{Victor Augusto Kich} % if too long for running head

\institute{
Victor Augusto Kich \and Alisson Henrique Kolling \and Daniel Fernando Tello Gamarra\at
Federal University of Santa Maria (UFSM)\newline
Santa Maria, RS, Brazil\newline
\email{victorkich@yahoo.com.br, alikolling@gmail.com, daniel.gamarra@ufsm.br}\and
Ricardo Bedin Grando \at 
Technological University of Uruguay (UTEC)\newline
Rivera, Uruguay\newline
\email{ricardo.bedin@utec.edu.uy}\and
Junior Costa de Jesus \and Paulo Lilles Jorge Drews-Jr \at
Federal University of Rio Grande (FURG)\newline
Rio Grande, RS, Brazil\newline
\email{dranaju@gmail.com, paulodrews@furg.br}
}

\date{Received: date / Accepted: date}

\date{Received: date / Accepted: date}
% The correct dates will be entered by the editor

% \maketitle

==> sections/6_methodology.tex <==
\section{Methodology}
\label{methodology}

